Routing Algorithms for Recursively-Defined Data Centre Networks

The server-centric data centre network architecture can accommodate a wide variety of network topologies. Newly proposed topologies in this arena often require several rounds of analysis and experimentation in order that they might achieve their full potential as data centre networks. We propose a family of novel routing algorithms on two well-known data centre networks of this type, (Generalized) DCell and FiConn, using techniques that can be applied more generally to the class of networks we call completely connected recursively-defined networks. In doing so, we develop a classification of all possible routes from server-node to server-node on these networks, called general routes of order $t$, and find that for certain topologies of interest, our routing algorithms efficiently produce paths that are up to 16% shorter than the best previously known algorithms, and are comparable to shortest paths. In addition to finding shorter paths, we show evidence that our algorithms also have good load-balancing properties.

==> plot_dcell_alpha_histograms.tex <==
% http://sourceforge.net/projects/pgfplots/
%\usepackage{pgfplots}
%\usetikzlibrary{patterns}
%\begin{document}
% Preamble: \pgfplotsset{width=7cm,compat=1.10} %\documentclass{article} %\usepackage{pgfplots} %\pgfplotsset{compat=1.5}
% \begin{document}

\begin{tikzpicture}
  \begin{axis}[width=\linewidth,
    % const plot mark left,
 %   small,
    height=5cm,
    ybar interval,
    xticklabel interval boundaries,
    xtick=data,
    x tick label style={rotate=90,anchor=east},
    %ybar, bar width=3pt,
%    ycomb,
%   title=Histogram of number of hops,
%   xlabel={No. of flows (intervals)},
   ylabel={Percent. of occurrence},
   legend entries={
     {\gp\gpi},
     {\dimr{}},
   },
   legend pos=north west,
%   grid=major,
%   mark=*,
%   mark fill = {blue, green, purple},
   ]

   % \addplot[fill=blue] table {dat/flow_hist_K3N10P0.0S.dat};
%\addplot[draw=blue] table {dat/knkstarK3N10P0_0S13219R4_hop_histogram.dat};
%\addplot[fill=purple] table {dat/flow_hist_K4N6P0.0S.dat};
%\addplot[fill=green] table {dat/flow_hist_ficonn_K2N24.dat};
   \addplot table
   {dat/ispa/histograms/DCell_beta_k3_clever_hist_k3n3t1000000s1norm.dat};%
   \addplot table
   {dat/ispa/histograms/DCell_beta_k3_clever_hist_k3n3t1000000splainnorm.dat};%
   
%\addplot[draw=purple] table {dat/knkstarK4N6P0.0S16331R4_hop_histogram.dat};
\end{axis}
\end{tikzpicture}
%\end{document}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SearchRouting"
%%% End:


==> plot_large_dcns.tex <==
% http://sourceforge.net/projects/pgfplots/
%\usepackage{pgfplots}
%\usetikzlibrary{patterns}
%\begin{document}
% Preamble: \pgfplotsset{width=7cm,compat=1.10} %\documentclass{article} %\usepackage{pgfplots} %\pgfplotsset{compat=1.5}
% \begin{document}

\begin{tikzpicture}
  \begin{axis}[width=\linewidth,
    sharp plot,
    % only marks,
    % point plot,
    ytick={0,1,2,3,4,5,6,7,8,9,10,11,12,13},
    xlabel={Alternatives attempted}, %
    ylabel={Percent savings},%
     xmin=-5,
     xmax=150,
     % minor x tick num = 100,
     legend entries={},
    % legend entries={%
    %   {\dcell\pms 3 {6}},{\gps\gpk{3}\gpi},%
    %   {\dcellb\pms 2 {43}},%{},%
    %   {\dcellb\pms 3 {6}},%,{\gps\gpk{3}\gpi},%
    %   {\ficonn\pms 3 {16}},{\gps\gpk{3}\gpi},%
    % },
    % legend to name=meanhops,
    % legend columns=-1,
    legend style={cells={anchor=west},font=\tiny,},
    legend pos=north east,
    grid=major,
    thin,
    mark size=1pt,
    ]
    \addplot[black,mark=diamond,] 
    table [x=alts,  y=percent]%
    {dat/ispa/DCell_alpha_k3k2_clever_k2n43t10000.dat};
    \addlegendentry[align=left]{
      \dcell\pms 2 {43}\\
      \gps\gpk{2}\gpi\gpr{r}
}

 %     \addplot[black,mark=diamond*,] 
 %     table [x=alts,  y=percent]%
 % {dat/ispa/DCell_alpha_k3k2_random_k2n43t10000.dat};


    % \addplot[black,mark=o,] 
    % table [x=alts,  y=percent]%
    % {dat/ispa/DCell_alpha_k3k2_clever_k3n6t10000.dat};
\addplot[black,mark=*,] 
    table [x=alts,  y=percent]%
    {dat/ispa/DCell_alpha_k3_clever_k3n6t10000.dat};
        \addlegendentry[align=left]{
      \dcell\pms 3 {6}\\
      \gps\gpk{3}\gpi\gpr{r}
}

    % \addplot[black,mark=*,] 
    % table [x=alts,  y=percent]%
    % {dat/ispa/DCell_alpha_k3_random_k3n6t10000.dat};

\addplot[black,mark=triangle,] 
    table [x=alts,  y=percent]%
    {dat/ispa/DCell_beta_k3k2_clever_k2n43t10000.dat};
    \addlegendentry[align=left]{
      \dcellb\pms 2 {43}\\
      \gps\gpk{2}\gpi\gpr{r}
}
    
%     \addplot[black,mark=triangle*,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_beta_k3k2_random_k2n43t10000.dat};

 %    \addplot[black,mark=pentagon,] 
 %    table [x=alts,  y=percent]%
 % {dat/ispa/DCell_beta_k3k2_clever_k3n6t10000.dat};
\addplot[black,mark=pentagon*,] 
    table [x=alts,  y=percent]%
    {dat/ispa/DCell_beta_k3_clever_k3n6t10000.dat};
        \addlegendentry[align=left]{
      \dcellb\pms 3 {6}\\
      \gps\gpk{3}\gpi\gpr{r}
}
    
    % \addplot[black,mark=*,] 
    % table [x=alts,  y=percent]%
    % {dat/ispa/DCell_beta_k3_random_k3n6t10000.dat};

    
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/FiConn_k3k2_clever_k3n16t10000.dat};
\addplot[black,mark=square*,] 
    table [x=alts,  y=percent]%
    {dat/ispa/FiConn_k3_clever_k3n16t10000.dat};
        \addlegendentry[align=left]{
      \ficonn\pms 3 {16}\\
      \gps\gpk{3}\gpi\gpr{r}
}
    
% \addplot[black,mark=square*,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/FiConn_k3_random_k3n16t10000.dat};

    % \addplot[black,mark=*,] 
    % table [x=alts,  y=percent]%
    % {dat/DCell_alpha_k3_clever_k3n6t10000.dat};
    % \addplot[red!70!black,mark=triangle*,] 
    % table [x=alts,  y=percent]%
    % {dat/DCell_alpha_k3_random_k3n6t10000.dat};
    % \addplot[blue,mark=square*,] 
    % table [x=alts,  y=percent]%
    % {dat/DCell_alpha_k3k2_clever_k3n6t10000.dat};
  \end{axis}
\end{tikzpicture}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SearchRouting"
%%% End:

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SearchRouting"
%%% End:


==> plot_large_random_dcns.tex <==
% http://sourceforge.net/projects/pgfplots/
%\usepackage{pgfplots}
%\usetikzlibrary{patterns}
%\begin{document}
% Preamble: \pgfplotsset{width=7cm,compat=1.10} %\documentclass{article} %\usepackage{pgfplots} %\pgfplotsset{compat=1.5}
% \begin{document}

\begin{tikzpicture}
  \begin{axis}[width=\linewidth,
    sharp plot,
    % only marks,
    % point plot,    
    ytick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14},
    xlabel={Number of proxy candidates}, %
    ylabel={Percent mean hop-length savings},%
%     xmin=-5,
     xmax=4000,
    % minor x tick num = 100,
    legend entries={%
      % {\dcell\pms 2 {43}},%
      % {\dcell\pms 3 {6}},{\gps\gpk{3}\gpk{2}\gpi},%
      % {\dcellb\pms 2 {43}},%
      % {\dcellb\pms 3 {6}},{\gps\gpk{3}\gpk{2}\gpi},%
      % {\ficonn\pms 3 {16}},{\gps\gpk{3}\gpk{2}\gpi},%%
    },
    % legend to name=meanhops,
    % legend columns=-1,
    legend style={cells={anchor=west},font=\tiny,},
    legend pos=north east,
    grid=both,
    thin,
    mark size=1pt,
    ]
%     \addplot[black,mark=diamond,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_alpha_k3k2_clever_k2n43t10000.dat};
     \addplot[black,mark=diamond*,] 
     table [x=alts,  y=percent]%
 {dat/ispa/DCell_alpha_k3k2_random_k2n43t10000.dat};
    \addlegendentry[align=left]{
      \dcell\pms 2 {43}\\
      \gps\gpk{2}\gpe\gpr{r}
}


% \addplot[black,mark=*,] 
%     table [x=alts,  y=percent]%
%     {dat/ispa/DCell_alpha_k3_clever_k3n6t10000.dat};
    \addplot[black,mark=*,] 
    table [x=alts,  y=percent]%
    {dat/ispa/DCell_alpha_k3_random_k3n6t10000.dat};
        \addlegendentry[align=left]{
      \dcell\pms 3 {6}\\
      \gps\gpk{3}\gpe\gpr{r}
}
     \addplot[black,mark=o,] 
     table [x=alts,  y=percent]%
     {dat/ispa/DCell_alpha_k3k2_clever_k3n6t10000.dat};
        \addlegendentry[align=left]{
      \dcell\pms 3 {6}\\
      \gps\gpk{3}\gpk{2}\gpi\gpr{r}
}

% \addplot[black,mark=triangle,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_beta_k3k2_clever_k2n43t10000.dat};
    \addplot[black,mark=triangle*,] 
    table [x=alts,  y=percent]%
{dat/ispa/DCell_beta_k3k2_random_k2n43t10000.dat};
    \addlegendentry[align=left]{
      \dcellb\pms 2 {43}\\
      \gps\gpk{2}\gpe\gpr{r}
}

% \addplot[black,mark=pentagon*,] 
%     table [x=alts,  y=percent]%
%     {dat/ispa/DCell_beta_k3_clever_k3n6t10000.dat};
    \addplot[black,mark=pentagon*,] 
    table [x=alts,  y=percent]%
    {dat/ispa/DCell_beta_k3_random_k3n6t10000.dat};
        \addlegendentry[align=left]{
      \dcellb\pms 3 {6}\\
      \gps\gpk{3}\gpe\gpr{r}
}
    \addplot[black,mark=pentagon,] 
    table [x=alts,  y=percent]%
 {dat/ispa/DCell_beta_k3k2_clever_k3n6t10000.dat};
        \addlegendentry[align=left]{
      \dcellb\pms 3 {6}\\
      \gps\gpk{3}\gpk{2}\gpi\gpr{r}
}
 
    
% \addplot[black,mark=square*,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/FiConn_k3_clever_k3n16t10000.dat};
\addplot[black,mark=square*,] 
    table [x=alts,  y=percent]%
{dat/ispa/FiConn_k3_random_k3n16t10000.dat};
        \addlegendentry[align=left]{
      \ficonn\pms 3 {16}\\
      \gps\gpk{3}\gpe\gpr{r}
}
     \addplot[black,mark=square,] 
     table [x=alts,  y=percent]%
 {dat/ispa/FiConn_k3k2_clever_k3n16t10000.dat};
        \addlegendentry[align=left]{
      \ficonn\pms 3 {16}\\
      \gps\gpk{3}\gpk{2}\gpi\gpr{r}
}

  \end{axis}
\end{tikzpicture}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SearchRouting"
%%% End:

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SearchRouting"
%%% End:


==> plot_small_dcns.tex <==
% http://sourceforge.net/projects/pgfplots/
%\usepackage{pgfplots}
%\usetikzlibrary{patterns}
%\begin{document}
% Preamble: \pgfplotsset{width=7cm,compat=1.10} %\documentclass{article} %\usepackage{pgfplots} %\pgfplotsset{compat=1.5}
% \begin{document}

\begin{tikzpicture}
  \begin{axis}[width=\linewidth,
    sharp plot,
    % only marks,
    % point plot,
    ytick={0,1,2,3,4,5},
    xlabel={Number of proxy candidates}, %
    ylabel={Percent mean hop-length savings},%
     xmin=-10,
     xmax=700,
    % minor x tick num = 100,
    legend entries={%
      % {\dcell\pms 2 {18}},{\gps\gpk{2}\gpe},%
      % {\dcellb\pms 2 {18}},{\gps\gpk{2}\gpe},%
      % {\ficonn\pms 2 {36}},{\gps\gpk{2}\gpe},%
      % {\ficonn\pms 3 {10}},{\gps\gpk{3}\gpi},{\gps\gpk{3}\gpe},%
    },
    % legend to name=meanhops,
    % legend columns=-1,
    legend style={cells={anchor=west},font=\tiny,},
    legend pos=north east,
    grid=both,
    thin,
    mark size=1pt,
    ]
    \addplot[black,mark=diamond,] 
    table [x=alts,  y=percent]%
{dat/ispa/DCell_alpha_k3k2_clever_k2n18t10000.dat};
    \addlegendentry[align=left]{
      \dcell\pms 2 {18}\\
      \gps\gpk{2}\gpi\gpr{r}
}
    \addplot[black,mark=diamond*,] 
    table [x=alts,  y=percent]%
{dat/ispa/DCell_alpha_k3k2_random_k2n18t10000.dat};
    \addlegendentry[align=left]{
      \dcell\pms 2 {43}\\
      \gps\gpk{2}\gpe\gpr{r}
}


\addplot[black,mark=triangle,] 
    table [x=alts,  y=percent]%
{dat/ispa/DCell_beta_k3k2_clever_k2n18t10000.dat};
    \addlegendentry[align=left]{
      \dcellb\pms 2 {18}\\
      \gps\gpk{2}\gpi\gpr{r}
}
    \addplot[black,mark=triangle*,] 
    table [x=alts,  y=percent]%
{dat/ispa/DCell_beta_k3k2_random_k2n18t10000.dat};
    \addlegendentry[align=left]{
      \dcellb\pms 2 {43}\\
      \gps\gpk{2}\gpe\gpr{r}
}



    \addplot[black,mark=square,] 
    table [x=alts,  y=percent]%
{dat/ispa/FiConn_k3k2_clever_k2n36t10000.dat};
    \addlegendentry[align=left]{
      \ficonn\pms 2 {36}\\
      \gps\gpk{2}\gpi\gpr{r}
}

\addplot[black,mark=square*,] 
    table [x=alts,  y=percent]%
{dat/ispa/FiConn_k2_random_k2n36t10000.dat};
    \addlegendentry[align=left]{
      \ficonn\pms 2 {36}\\
      \gps\gpk{2}\gpe\gpr{r}
}


    \addplot[black,mark=o,] 
    table [x=alts,  y=percent]%
    {dat/ispa/FiConn_k3k2_clever_k3n10t10000.dat};
    \addlegendentry[align=left]{
      \ficonn\pms 3 {10}\\
      \gps\gpk{3}\gpk{2}\gpi\gpr{r}
}
    
\addplot[black,mark=oplus,] 
    table [x=alts,  y=percent]%
{dat/ispa/FiConn_k3_clever_k3n10t10000.dat};
    \addlegendentry[align=left]{
      \ficonn\pms 3 {10}\\
      \gps\gpk{3}\gpi\gpr{r}
}

\addplot[black,mark=*,] 
    table [x=alts,  y=percent]%
{dat/ispa/FiConn_k3_random_k3n10t10000.dat};
    \addlegendentry[align=left]{
      \ficonn\pms 3 {10}\\
      \gps\gpk{3}\gpe\gpr{r}
}


%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/FiConn_k3_clever_k3n16t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/FiConn_k3k2_clever_k3n16t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_beta_k3k2_random_k2n43t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_beta_k3k2_clever_k2n43t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_beta_k3k2_clever_k3n6t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_alpha_k3k2_random_k2n43t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_beta_k3_clever_k3n6t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_beta_k3_random_k3n6t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_alpha_k3k2_clever_k2n43t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_alpha_k3k2_clever_k3n6t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_alpha_k3_clever_k3n6t10000.dat};
%     \addplot[black,mark=square,] 
%     table [x=alts,  y=percent]%
% {dat/ispa/DCell_alpha_k3_random_k3n6t10000.dat};


    % \addplot[black,mark=*,] 
    % table [x=alts,  y=percent]%
    % {dat/DCell_alpha_k3_clever_k3n6t10000.dat};
    % \addplot[red!70!black,mark=triangle*,] 
    % table [x=alts,  y=percent]%
    % {dat/DCell_alpha_k3_random_k3n6t10000.dat};
    % \addplot[blue,mark=square*,] 
    % table [x=alts,  y=percent]%
    % {dat/DCell_alpha_k3k2_clever_k3n6t10000.dat};
  \end{axis}
\end{tikzpicture}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SearchRouting"
%%% End:

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SearchRouting"
%%% End:

